From Lazy to Prolific: Tackling Missing Labels in Open Vocabulary Extreme Classification by Positive-Unlabeled Sequence Learning

Open-vocabulary Extreme Multi-label Classification (OXMC) extends traditional XMC by allowing prediction beyond an extremely large, predefined label set (typically $10^3$ to $10^{12}$ labels), addressing the dynamic nature of real-world labeling tasks. However, self-selection bias in data annotation leads to significant missing labels in both training and test data, particularly for less popular inputs. This creates two critical challenges: generation models learn to be "lazy'" by under-generating labels, and evaluation becomes unreliable due to insufficient annotation in the test set. In this work, we introduce Positive-Unlabeled Sequence Learning (PUSL), which reframes OXMC as an infinite keyphrase generation task, addressing the generation model's laziness. Additionally, we propose to adopt a suite of evaluation metrics, F1@$\mathcal{O}$ and newly proposed B@$k$, to reliably assess OXMC models with incomplete ground truths. In a highly imbalanced e-commerce dataset with substantial missing labels, PUSL generates 30% more unique labels, and 72% of its predictions align with actual user queries. On the less skewed EURLex-4.3k dataset, PUSL demonstrates superior F1 scores, especially as label counts increase from 15 to 30. Our approach effectively tackles both the modeling and evaluation challenges in OXMC with missing labels.

==> 4-exp_gini_index.tex <==
\subsection{Impact analysis of PUSL}

Graph of Gini Index. x-axis is the cumulative proportion of item, y-axis is cumulative propotion of the keyphrase.

The surplus area in the gini graph is the impact of the PUSL model. It increases the total number of keyphrase by significant amount. 

Compare the area of PUSL with Groundthruth and Uniform Keyphrase.

More keyphrase more revenue.

need to cite this post\footnote{\url{https://neuroplausible.com/gini}}
\input{tables/gini}

==> X-bias_of_baselines.tex <==

\subsection{Bias in Existing Models}
\haoran{Shrink and move the bias content to the baseline section.}
% \haoran{Introduce the 80/20 rule and a small figure, and our model aims to flatten the num of kp curve to k. Shrink and move the bias content to the baseline section.}
% \subsection{Bias of Existing Keyphrase Generation Paradigms}


\paragraph{One2Seq:} The One2Seq paradigm \cite{chan2019neural,yuan-etal-2020-one} treats keyphrase generation as a sequence generation task. The target keyphrases are sorted in a predefined order and concatenated into a single sequence, with delimiters (<sep>) separating individual keyphrases and an end-of-sequence (EOS, </s>) token at the end. During training, the model learns to generate the entire keyphrase sequence given the input document and to self-terminate by generating the EOS token when all ground truth keyphrases have been exhausted. At inference time, the model generates a sequence of keyphrases, which are then split based on the delimiters to obtain the final set of predicted keyphrases.

Figure~\ref{fig:catseq} illustrates the decoding transition diagram of the One2Seq paradigm. 
When training a One2Seq model with incomplete XMC data, 
the model may prematurely generate the EOS token (bias: $\text{kp token} \rightarrow \text{</s>}$), leading to shorter keyphrase sequences and failing to capture the full range of possible keyphrases for a given document. 
% the probability of the EOS token tends to increase as the decoding length grows. 
This correlation may be spurious due to the absence of the majority of rare-long data points in the training set. If the training data were complete, the model would likely learn to generate more keyphrases per document, resulting in longer decoding sequences until EOS.



\paragraph{One2One:} In the One2One paradigm \cite{meng-etal-2017-deep,chen-etal-2019-integrated,Chen_Gao_Zhang_King_Lyu_2019}, each training instance consists of an input document and a single corresponding keyphrase from the set of target keyphrases. During inference, One2One models employ beam search to generate candidate keyphrases and select the top-$K$ ranked ones as the final keyphrases.

In XMC task, the problem arises from the long-tailed keyphrase distribution, where different keyphrases may compete to be the only ground truth. At the end, the common keyphrase tends to be fully trained while the rare keyphrase is less encouraged during the training (bias: $\text{<s>} \rightarrow \text{kp token}$ \rui{this bias is not very clear to me.}\haoran{Need to find some paper}) in Figure~\ref{fig:one2one}. 

One2Set \cite{ye-etal-2021-one2set} employs paralleled decoding on top of One2One, which potentially mitigates the keyphrase competing problem, but they also expect the model to learn to self-terminate by generating EOS directly after the BOS token. As studied in \cite{xie2022wr}, the One2Set also tends to generate excessive empty keyphrases (bias: $\text{<s>} \rightarrow \text{</s>}$, Figure~\ref{fig:one2one}).


==> X-meeting_notes.tex <==
\section{Meeting Notes}

==> X-paper_notes.tex <==
\section{Paper Notes}
\subsection{Theory}

\begin{itemize}
    \item (this is about evaluation, not theory) Beyond Standard Performance Measures in Extreme Multi-label Classification \cite{schultheis2022beyond}
    \item On Missing Labels, Long-tails and Propensities in Extreme Multi-label Classification \cite{schultheis2022missing}
    \item SiameseXML: Siamese Networks meet Extreme Classifiers with 100M Labels \cite{dahiya2021siamesexml} \url{https://www.cse.iitk.ac.in/users/purushot/papers/siamesexml_supp.pdf}
    \item (rejected theory paper) Unbiased Estimates for Multilabel Reductions of Extreme Classification with Missing Labels \url{https://openreview.net/forum?id=9zWlrwlT9-j}
    \item Long-tailed Extreme Multi-label Text Classification by the Retrieval of Generated Pseudo Label Descriptions \cite{zhang-etal-2023-long}
    \item Theoretical Comparisons of Positive-Unlabeled Learning against Positive-Negative Learning \cite{niu2016theoretical}
    \item Multi-Positive and Unlabeled Learning \cite{xu2017multi}
\end{itemize}

\subsection{NLP}

\begin{itemize}
    \item Pretrained generalized autoregressive model with adaptive probabilistic label clusters for extreme multi-label text classification \cite{ye2020pretrained}
    \item Open Vocabulary Extreme Classification Using Generative Models 
    \item Cluster-Guided Label Generation in Extreme Multi-Label Classification
\end{itemize}

==> introduction_alternate.tex <==
\section{Introduction-soumik}
In the space of advertisement, the sponsored search mechanism~\cite{jansen2008sponsored} enables promotion of entities on the search results page (SRPs). While search provides a platform for buyers to navigate the huge inventory of items listed by the sellers, advertisement enables sellers to promote their entities which might get lost otherwise in the vast ocean of search traffic driving sales/hits for their promoted entities. Key-phrase targeting is provided to sellers as a feature of advertisement, to target the buyer queries providing the sellers buyer outreach and sales traction. Query (or key-phrase) recommendations are generally made from titles of e-commerce products, product descriptions, transcripts of promotional videos, posts on social media sites, and other search-based platforms using sponsored entities~\cite{bartz2006logistic,yih2006finding}. 

On e-commerce platforms such as Amazon, eBay, and Walmart, sellers are recommended key-phrases based on their inventory listing's metadata. For instance, a seller may have a listing titled ``New iPhone 15 Pro Max 128 GB White" in the Electronics category. We seek to develop a recommender algorithm that will generate a relevant collection of key-phrases such as ``latest iphone", ``128 gb iphone 15", ``new iphone", ``apple phone 15", or even ``latest Samsung smartphone.'' We use \emph{key-phrase} instead of the more common keyword in this paper to indicate that a phrase can have multiple words; also, the ordering of words in the phrase matters. The listing length in words is typically very low, and the key-phrase may contain words that do not even occur in the listing. 

Conventionally, logs generated by search engine responses \cite{aglo2000QueryLog,bartz2006logistic} to buyer queries have been the data source for recommendation systems. This helps to associate key-phrases that are not only relevant to the products, but are also actively searched by buyers. We have provided more details on the data generation process in Section~\ref{ss:dataset_gen}.It is important for key-phrase recommendation in the advertisement space to have key-phrases which are search queries for targeting purposes, i.e., when advertisers want to bid on said key-phrases, these are actual queries and not queries that seem plausible but non-existent. Since the nature of the problem is mapping items to \emph{multiple} queries to increase the potential reach of the advertisers, this problem of key-phrase recommendation can be formulated as an Extreme Multi-Label (XML) Classification problem. Key-phrase recommendation has been explored using query-query similarity with click graphs~\cite{antonellis2008simrank++}, and formulated as an XML problem in~\cite{agrawal2013multi}.

Aggregated data from the logs typically contains billions of data points due to the large number of key-phrases and the buyer activity associated. In addition, the buyer behavior tends to favor certain \textit{popular items}, which appear organically in the search algorithm due to the items being associated with more queries and buyer activity. The phenomenon of most items not being mapped to its full potential of query outreach  is heavily influenced not only by buyer activity but also from the search algorithm bias which is influenced by the said activity --- making this a catch-22 situation. 

In the domain of advertisement, our main aim is to disrupt this cycle of bias by connecting less popular items to its full potential of queries by creating an avenue for promotion, subverting the original flow of the search algorithm --- and subsequently influencing buyer behavior by creating impressions/clicks for these promoted items. The interaction of search and advertisement forms a complex dynamical system, where search caters to buyer activity and has it's own definition of relevance and ranking based on buyer side metrics, while ads interact with search by adhering to search's definition of relevance and exerting influence on search's ranking through promotion. This creates a unique challenge for XMC where it's important for algorithms to be label-aware i.e., learn how queries tend to be typically in the platform, and relevant (according to search) to the seed-item --- while at the same time making every item reach it's fullest potential in terms of keywords (buyer outreach) even in the absence of said mappings in the training set.

%We look into the problem of suggesting keyphrases for a new listing put by a seller based on the words in its title. While a seller might provide additional information about the listing such as categorization, brand and so on, he or she constructs the title accurate enough to attract buyers. The suggestion needs to be made while the seller is creating the listing. There are two ways to solve this problem, either by suggesting existing keyphrases based on similar listing associations which we term as \emph{keyphrase recommendation}, or by constructing valid keyphrases from words in the listing's title termed as  \emph{keyphrase generation}. We focus on the first problem in this paper. A brute way to solve the problem is by comparing the new listing's title to that of all the existing listings and return the corresponding listing's keyphrases upon closest match. However, this process will be expensive owing to the large number of listed products. An efficient solution requires recommendations in real-time and use of resources in a constrained manner. Besides, the issue of \emph{cold start} where newer listings that have never been created on the platform still remains. Also, it would be productive to look for keyphrases within each product category, thus building a model per category is essential for good accuracy.%

% The following features are desired for ideal keyphrase suggestions to the seller:
% \begin{enumerate}
%     \item Consistency: Different listings for the same product should have identical keyphrases. This is to ensure fairness across sellers and doesn't disadvantage certain sellers.
%     \item Sensitivity: Certain words in the keyphrases might have more impact than others and should thus be included in the recommendation. Ex, gender specific words might be more important to the customer when looking for a product.
%     \item Interpretability: The model's recommendations should be explainable as to why it was predicted. Determining whether certain recommendations are incorrect is essential.
%     \item Diversity: The keyphrases recommended for a particular listing are different and not simple re-orderings of each other.
%     \item Quantity: A large number of recommendations are required to made which provides more options to the seller.
%     \item Fast: Recommendations should be made in real-time.
% \end{enumerate}

==> tables/ablation_ppusl.tex <==
\begin{table}[!t]
\centering
% \scriptsize
\footnotesize
\begin{tabular}{@{}l|rrrrr@{}}
\toprule
Model & \#K@$\mu$ & \#K@$2\mu$ & B@$\mu$ & B@$2\mu$ & F1@$\mathcal{O}$ \\ \midrule
\multicolumn{6}{c}{Test-Narrow ($|\mathcal{Y}| \leq 2\mu$)} \\ \midrule
PUSL w/o PT & 2.46 & 3.31 & \textbf{34.50} & \textbf{19.48} & \textbf{38.54} \\
PUSL w/ \ \ PT& \textbf{2.52} & \textbf{3.44} & 32.39 & 18.51 & 35.75 \\ \midrule
\multicolumn{6}{c}{Test-Diverse ($|\mathcal{Y}| > 2\mu$)} \\ \midrule
PUSL w/o PT & 2.46 & 3.23 & \textbf{56.14} & \textbf{33.79} & \textbf{27.94} \\
PUSL w/ \ \ PT& \textbf{2.49} & \textbf{3.34} & 55.49 & 33.44 & 25.65 \\
\bottomrule
\end{tabular}
\caption{Ablation study on PUSL with and without post-training. }
\label{tab:ppusl_ablation}
\end{table}

==> tables/annotator_example.tex <==
\begin{table*}[!htbp]
\centering
\begin{tabularx}{\textwidth}{|l|X|}
\hline
\textbf{Item Description} & MaxMara coat wool trench coat \\
\hline
\textbf{Annotator(s)} &  \\
\hline
1 Lazy & winter coat \\
\hline
1 Hard-working & winter coat, coat, wool coat, fall coat, trench coat, luxury coat \\
\hline
N Lazy & winter coat, coat \\
\hline
N Hard-working & winter coat, coat, fur coat, wool coat, fall coat, cashmere coat, faux fur coat, teddy bear coat, sterling coat, designers coat, high-end coat, luxury coat, trench coat, alpaca coat, wool blend coat, camel coat, wool \& cashmere coat ...\\
\hline
\end{tabularx}
\caption{Annotation results for different types and numbers of annotators}
\label{tab:maxmara}
\end{table*}


==> tables/budgetk.tex <==
\begin{table*}[]
% \label{Table:perf-comparison}
\centering
% \small
\scriptsize
\begin{tabular}{l|llllllllllll}
\toprule
& \multicolumn{12}{c}{AmazonCat} \\ \midrule
& \multicolumn{4}{l|}{Short ($|\mathcal{Y}| \leq 3$)} & \multicolumn{4}{l|}{Medium ($ 4 \leq |\mathcal{Y}| \leq 9$)} & \multicolumn{4}{l}{Long ($ 10 \leq |\mathcal{Y}|$)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{6} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{6} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l}{6} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule
GROOV & \multicolumn{1}{l}{73.0} & \multicolumn{1}{l|}{78.2} & \multicolumn{1}{l}{72.0} & \multicolumn{1}{l|}{78.5} & \multicolumn{1}{l}{88.5} & \multicolumn{1}{l|}{39.1} & \multicolumn{1}{l}{86.4} & \multicolumn{1}{l|}{45.8} & \multicolumn{1}{l}{92.0} & \multicolumn{1}{l|}{19.6} & \multicolumn{1}{l}{89.3} & \multicolumn{1}{l}{24.3}\\ 
One2Seq (correct) & \multicolumn{1}{l}{19.1} & \multicolumn{1}{l|}{33.6} & \multicolumn{1}{l}{17.7} & \multicolumn{1}{l|}{56.7} & \multicolumn{1}{l}{63.8} & \multicolumn{1}{l|}{30.4} & \multicolumn{1}{l}{53.8} & \multicolumn{1}{l|}{50.9} & \multicolumn{1}{l}{78.7} & \multicolumn{1}{l|}{18.1} & \multicolumn{1}{l}{70.7} & \multicolumn{1}{l}{32.4}\\ 
One2Seq (no eos) & \multicolumn{1}{l}{24.4} & \multicolumn{1}{l|}{34.5} & \multicolumn{1}{l}{19.7} & \multicolumn{1}{l|}{57.5} & \multicolumn{1}{l}{67.6} & \multicolumn{1}{l|}{32.8} & \multicolumn{1}{l}{56.9} & \multicolumn{1}{l|}{54.9} & \multicolumn{1}{l}{78.5} & \multicolumn{1}{l|}{18.0} & \multicolumn{1}{l}{69.3} & \multicolumn{1}{l}{31.8}\\ 


One2One & \multicolumn{1}{l}{24.4} & \multicolumn{1}{l|}{34.5} & \multicolumn{1}{l}{19.7} & \multicolumn{1}{l|}{57.5} & \multicolumn{1}{l}{67.6} & \multicolumn{1}{l|}{32.8} & \multicolumn{1}{l}{56.9} & \multicolumn{1}{l|}{54.9} & \multicolumn{1}{l}{78.5} & \multicolumn{1}{l|}{18.0} & \multicolumn{1}{l}{68.3} & \multicolumn{1}{l}{31.8}\\ 
PUSL & \multicolumn{1}{l}{22.2} & \multicolumn{1}{l|}{38.3} & \multicolumn{1}{l}{20.9} & \multicolumn{1}{l|}{63.7} & \multicolumn{1}{l}{65.0} & \multicolumn{1}{l|}{31.0} & \multicolumn{1}{l}{57.1} & \multicolumn{1}{l|}{52.5} & \multicolumn{1}{l}{79.2} & \multicolumn{1}{l|}{18.2} & \multicolumn{1}{l}{71.5} & \multicolumn{1}{l}{32.7}\\ \midrule
& \multicolumn{12}{c}{Wikipedia-1M} \\ \midrule
& \multicolumn{4}{l|}{Short ($|\mathcal{Y}| \leq 4$)} & \multicolumn{4}{l|}{Medium ($ 5 \leq |\mathcal{Y}| \leq 10$)} & \multicolumn{4}{l}{Long ($ 11 \leq |\mathcal{Y}|$)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{2} & \multicolumn{2}{l|}{4} & \multicolumn{2}{l|}{2} & \multicolumn{2}{l|}{4} & \multicolumn{2}{l|}{2} & \multicolumn{2}{l}{4} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule
GROOV & \multicolumn{1}{l}{62.8} & \multicolumn{1}{l|}{48.3} & \multicolumn{1}{l}{61.2} & \multicolumn{1}{l|}{51.6} & \multicolumn{1}{l}{80.7} & \multicolumn{1}{l|}{25.7} & \multicolumn{1}{l}{75.4} & \multicolumn{1}{l|}{36.1} & \multicolumn{1}{l}{92.3} & \multicolumn{1}{l|}{13.8} & \multicolumn{1}{l}{85.9} & \multicolumn{1}{l}{23.0}\\ 
One2Seq (correct) & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l}{42.2}\\ 
One2Seq (no eos) & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l}{42.2}\\ 
One2One & \multicolumn{1}{l}{40.3} & \multicolumn{1}{l|}{36.4} & \multicolumn{1}{l}{29.1} & \multicolumn{1}{l|}{50.6} & \multicolumn{1}{l}{62.5} & \multicolumn{1}{l|}{19.2} & \multicolumn{1}{l}{53.2} & \multicolumn{1}{l|}{32.6} & \multicolumn{1}{l}{75.0} & \multicolumn{1}{l|}{10.5} & \multicolumn{1}{l}{68.5} & \multicolumn{1}{l}{19.1}\\ 
PUSL & \multicolumn{1}{l}{19.3} & \multicolumn{1}{l|}{13.4} & \multicolumn{1}{l}{15.3} & \multicolumn{1}{l|}{17.1} & \multicolumn{1}{l}{54.6} & \multicolumn{1}{l|}{16.1} & \multicolumn{1}{l}{39.4} & \multicolumn{1}{l|}{21.1} & \multicolumn{1}{l}{75.7} & \multicolumn{1}{l|}{10.5} & \multicolumn{1}{l}{60.4} & \multicolumn{1}{l}{15.8}\\ \midrule
& \multicolumn{12}{c}{EURLex4.3k} \\ \midrule
& \multicolumn{4}{l|}{Short ($|\mathcal{Y}| \leq 14$)} & \multicolumn{4}{l|}{Medium ($ 15 \leq |\mathcal{Y}| \leq 28$)} & \multicolumn{4}{l}{Long ($ 29 \leq |\mathcal{Y}|$)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{10} & \multicolumn{2}{l|}{20} & \multicolumn{2}{l|}{10} & \multicolumn{2}{l|}{20} & \multicolumn{2}{l|}{10} & \multicolumn{2}{l}{20} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule
GROOV & \multicolumn{1}{l}{57.7} & \multicolumn{1}{l|}{35.7} & \multicolumn{1}{l}{57.4} & \multicolumn{1}{l|}{36.0} & \multicolumn{1}{l}{55.9} & \multicolumn{1}{l|}{20.2} & \multicolumn{1}{l}{54.7} & \multicolumn{1}{l|}{20.9} & \multicolumn{1}{l}{74.8} & \multicolumn{1}{l|}{18.6} & \multicolumn{1}{l}{70.7} & \multicolumn{1}{l}{28.4}\\ 
One2Seq (correct) & \multicolumn{1}{l}{52.1} & \multicolumn{1}{l|}{54.3} & \multicolumn{1}{l}{37.9} & \multicolumn{1}{l|}{72.1} & \multicolumn{1}{l}{71.1} & \multicolumn{1}{l|}{37.8} & \multicolumn{1}{l}{61.2} & \multicolumn{1}{l|}{62.8} & \multicolumn{1}{l}{71.0} & \multicolumn{1}{l|}{19.4} & \multicolumn{1}{l}{80.0} & \multicolumn{1}{l}{43.8}\\ 
One2Seq (no eos) & \multicolumn{1}{l}{50.9} & \multicolumn{1}{l|}{53.1} & \multicolumn{1}{l}{36.5} & \multicolumn{1}{l|}{74.0} & \multicolumn{1}{l}{69.3} & \multicolumn{1}{l|}{36.9} & \multicolumn{1}{l}{59.5} & \multicolumn{1}{l|}{62.6} & \multicolumn{1}{l}{75.0} & \multicolumn{1}{l|}{20.6} & \multicolumn{1}{l}{82.2} & \multicolumn{1}{l}{45.3}\\ 
One2One & \multicolumn{1}{l}{40.9} & \multicolumn{1}{l|}{41.8} & \multicolumn{1}{l}{29.5} & \multicolumn{1}{l|}{60.2} & \multicolumn{1}{l}{57.6} & \multicolumn{1}{l|}{30.7} & \multicolumn{1}{l}{44.2} & \multicolumn{1}{l|}{47.1} & \multicolumn{1}{l}{44.6} & \multicolumn{1}{l|}{12.3} & \multicolumn{1}{l}{32.6} & \multicolumn{1}{l}{18.1}\\ 
PUSL & \multicolumn{1}{l}{52.6} & \multicolumn{1}{l|}{55.3} & \multicolumn{1}{l}{41.6} & \multicolumn{1}{l|}{75.5} & \multicolumn{1}{l}{71.3} & \multicolumn{1}{l|}{37.9} & \multicolumn{1}{l}{64.4} & \multicolumn{1}{l|}{64.8} & \multicolumn{1}{l}{85.7} & \multicolumn{1}{l|}{23.7} & \multicolumn{1}{l}{87.0} & \multicolumn{1}{l}{47.8}\\ \midrule
& \multicolumn{12}{c}{eBay} \\ \midrule
& \multicolumn{4}{l|}{Short ($|\mathcal{Y}| \leq 3$)} & \multicolumn{4}{l|}{Medium ($ 4 \leq |\mathcal{Y}| \leq 5$)} & \multicolumn{4}{l}{Long ($ 6 \leq |\mathcal{Y}|)$} \\ \midrule
Budget@k & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{5} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{5} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l}{5} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule
GROOV & \multicolumn{1}{l}{48.0} & \multicolumn{1}{l|}{27.1} & \multicolumn{1}{l}{48.0} & \multicolumn{1}{l|}{27.1} & \multicolumn{1}{l}{64.2} & \multicolumn{1}{l|}{14.2} & \multicolumn{1}{l}{64.2} & \multicolumn{1}{l|}{14.2} & \multicolumn{1}{l}{73.3} & \multicolumn{1}{l|}{7.0} & \multicolumn{1}{l}{73.3} & \multicolumn{1}{l}{7.0}\\ 
One2Seq (correct) & \multicolumn{1}{l}{25.9} & \multicolumn{1}{l|}{40.1} & \multicolumn{1}{l}{19.7} & \multicolumn{1}{l|}{43.5} & \multicolumn{1}{l}{42.3} & \multicolumn{1}{l|}{26.7} & \multicolumn{1}{l}{32.2} & \multicolumn{1}{l|}{29.6} & \multicolumn{1}{l}{56.2} & \multicolumn{1}{l|}{14.3} & \multicolumn{1}{l}{44.7} & \multicolumn{1}{l}{16.6}\\ 
One2Seq (no eos) & \multicolumn{1}{l}{15.9} & \multicolumn{1}{l|}{46.8} & \multicolumn{1}{l}{11.9} & \multicolumn{1}{l|}{50.0} & \multicolumn{1}{l}{36.8} & \multicolumn{1}{l|}{31.5} & \multicolumn{1}{l}{28.1} & \multicolumn{1}{l|}{34.8} & \multicolumn{1}{l}{56.2} & \multicolumn{1}{l|}{14.3} & \multicolumn{1}{l}{44.7} & \multicolumn{1}{l}{16.6}\\ 
One2One & \multicolumn{1}{l}{27.1} & \multicolumn{1}{l|}{42.7} & \multicolumn{1}{l}{20.1} & \multicolumn{1}{l|}{51.9} & \multicolumn{1}{l}{45.3} & \multicolumn{1}{l|}{28.9} & \multicolumn{1}{l}{36.2} & \multicolumn{1}{l|}{38.5} & \multicolumn{1}{l}{59.6} & \multicolumn{1}{l|}{15.5} & \multicolumn{1}{l}{51.7} & \multicolumn{1}{l}{22.1}\\ 
PUSL & \multicolumn{1}{l}{31.8} & \multicolumn{1}{l|}{45.6} & \multicolumn{1}{l}{27.1} & \multicolumn{1}{l|}{49.2} & \multicolumn{1}{l}{51.1} & \multicolumn{1}{l|}{30.2} & \multicolumn{1}{l}{45.6} & \multicolumn{1}{l|}{34.5} & \multicolumn{1}{l}{66.5} & \multicolumn{1}{l|}{16.0} & \multicolumn{1}{l}{61.4} & \multicolumn{1}{l}{19.1}\\


\bottomrule
\end{tabular}
% \label{tab:main}
\caption{Evaluation on budget@k. We split Short, Medium, Long by <=50, >50 and =<90, >90 quantile.\haoran{change these to narrow, medium, diverse}\haoran{We cannot run faithful evaluation on the narrow split due to incomplete ground truth, but the scores on diverse set could be a good approximation}\haoran{I want to use both bold text and cell highlight.}}
\end{table*}



% \begin{table*}[]
% \centering
% \scriptsize
% \begin{tabular}{|l|llllllllllllllllll|}
% \hline
%            & \multicolumn{6}{l|}{Short}                                                                                                                                            & \multicolumn{6}{l|}{Medium}                                                                                                                                           & \multicolumn{6}{l|}{Long}                                                                                                                        \\ \hline
%            & \multicolumn{18}{l|}{AmazonCat}                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
% k          & \multicolumn{3}{l|}{5}                                                            & \multicolumn{3}{l|}{10}                                                           & \multicolumn{3}{l|}{5}                                                            & \multicolumn{3}{l|}{10}                                                           & \multicolumn{3}{l|}{5}                                                            & \multicolumn{3}{l|}{10}                                      \\ \hline
%            & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & F    \\ \hline
% PUSL       & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & 42.2 \\ \hline
% DS(o2o)    & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     &      \\ \hline
% GROOV      & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     &      \\ \hline
% DS(catseq) & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     &      \\ \hline
% \end{tabular}
% \end{table*}

==> tables/budgetk_modified.tex <==
\begin{table*}[t]
% \label{Table:perf-comparison}
\centering
% \small
\scriptsize
\begin{tabular}{l|llllllllllll}
\toprule
& \multicolumn{12}{c}{AmazonCat} \\ \midrule
& \multicolumn{4}{l|}{Narrow ($|\mathcal{Y}| \leq 3$) (placeholder\%)} & \multicolumn{4}{l|}{Medium ($ 4 \leq |\mathcal{Y}| \leq 9$) (placeholder\%)} & \multicolumn{4}{l}{Diverse ($ 10 \leq |\mathcal{Y}|$) (placeholder\%)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{6} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{6} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l}{6} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule
GROOV & \multicolumn{1}{l}{50.6} & \multicolumn{1}{l|}{78.2} & \multicolumn{1}{l}{25.4} & \multicolumn{1}{l|}{78.5} & \multicolumn{1}{l}{79} & \multicolumn{1}{l|}{39.1} & \multicolumn{1}{l}{46.6} & \multicolumn{1}{l|}{45.8} & \multicolumn{1}{l}{84.8} & \multicolumn{1}{l|}{19.6} & \multicolumn{1}{l}{52.8} & \multicolumn{1}{l}{24.3}\\ 
One2Seq (correct) & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l}-\\ 
% One2Seq (no eos) & \multicolumn{1}{l}{18.8} & \multicolumn{1}{l|}{33.2} & \multicolumn{1}{l}{16.8} & \multicolumn{1}{l|}{54.6} & \multicolumn{1}{l}{63.0} & \multicolumn{1}{l|}{29.9} & \multicolumn{1}{l}{52.0} & \multicolumn{1}{l|}{48.9} & \multicolumn{1}{l}{78.6} & \multicolumn{1}{l|}{18.1} & \multicolumn{1}{l}{70.5} & \multicolumn{1}{l}{32.3}\\ 


One2One & \multicolumn{1}{l}{24.4} & \multicolumn{1}{l|}{34.5} & \multicolumn{1}{l}{19.7} & \multicolumn{1}{l|}{57.5} & \multicolumn{1}{l}{67.6} & \multicolumn{1}{l|}{32.8} & \multicolumn{1}{l}{56.9} & \multicolumn{1}{l|}{54.8} & \multicolumn{1}{l}{78.5} & \multicolumn{1}{l|}{18.0} & \multicolumn{1}{l}{69.3} & \multicolumn{1}{l}{31.8}\\ 
PUSL & \multicolumn{1}{l}{21.7} & \multicolumn{1}{l|}{37.6} & \multicolumn{1}{l}{20} & \multicolumn{1}{l|}{63.7} & \multicolumn{1}{l}{64.6} & \multicolumn{1}{l|}{30.7} & \multicolumn{1}{l}{55.4} & \multicolumn{1}{l|}{52.5} & \multicolumn{1}{l}{79.1} & \multicolumn{1}{l|}{18.2} & \multicolumn{1}{l}{71.5} & \multicolumn{1}{l}{32.7}\\ \midrule
& \multicolumn{12}{c}{Wikipedia-1M} \\ \midrule
& \multicolumn{4}{l|}{Narrow ($|\mathcal{Y}| \leq 4$)} & \multicolumn{4}{l|}{Medium ($ 5 \leq |\mathcal{Y}| \leq 10$)} & \multicolumn{4}{l}{Diverse ($ 11 \leq |\mathcal{Y}|$)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{2} & \multicolumn{2}{l|}{4} & \multicolumn{2}{l|}{2} & \multicolumn{2}{l|}{4} & \multicolumn{2}{l|}{2} & \multicolumn{2}{l}{4} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule
GROOV & \multicolumn{1}{l}{51.6} & \multicolumn{1}{l|}{48.3} & \multicolumn{1}{l}{28.5} & \multicolumn{1}{l|}{51.6} & \multicolumn{1}{l}{79.1} & \multicolumn{1}{l|}{25.7} & \multicolumn{1}{l}{56.7} & \multicolumn{1}{l|}{36.1} & \multicolumn{1}{l}{92.1} & \multicolumn{1}{l|}{13.8} & \multicolumn{1}{l}{77.6} & \multicolumn{1}{l}{23.0}\\ 
One2Seq (correct) & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l}{42.2}\\ 
% One2Seq (no eos) & \multicolumn{1}{l}{20.6} & \multicolumn{1}{l|}{16.3} & \multicolumn{1}{l}{13.1} & \multicolumn{1}{l|}{20.9} & \multicolumn{1}{l}{55.9} & \multicolumn{1}{l|}{16.8} & \multicolumn{1}{l}{37.5} & \multicolumn{1}{l|}{22.4} & \multicolumn{1}{l}{77.0} & \multicolumn{1}{l|}{10.8} & \multicolumn{1}{l}{59.8} & \multicolumn{1}{l}{16.6}\\ 
One2One & \multicolumn{1}{l}{40.3} & \multicolumn{1}{l|}{36.4} & \multicolumn{1}{l}{29.0} & \multicolumn{1}{l|}{50.5} & \multicolumn{1}{l}{62.5} & \multicolumn{1}{l|}{19.2} & \multicolumn{1}{l}{53.1} & \multicolumn{1}{l|}{32.6} & \multicolumn{1}{l}{75.0} & \multicolumn{1}{l|}{10.5} & \multicolumn{1}{l}{68.5} & \multicolumn{1}{l}{19.1}\\ 
PUSL & \multicolumn{1}{l}{17.3} & \multicolumn{1}{l|}{13.3} & \multicolumn{1}{l}{11.1} & \multicolumn{1}{l|}{17.1} & \multicolumn{1}{l}{53.3} & \multicolumn{1}{l|}{16.0} & \multicolumn{1}{l}{35.3} & \multicolumn{1}{l|}{21.1} & \multicolumn{1}{l}{74.8} & \multicolumn{1}{l|}{10.5} & \multicolumn{1}{l}{57.1} & \multicolumn{1}{l}{15.8}\\ \midrule
& \multicolumn{12}{c}{EURLex4.3k} \\ \midrule
& \multicolumn{4}{l|}{Narrow ($|\mathcal{Y}| \leq 14$)} & \multicolumn{4}{l|}{Medium ($ 15 \leq |\mathcal{Y}| \leq 28$)} & \multicolumn{4}{l}{Diverse ($ 29 \leq |\mathcal{Y}|$)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{10} & \multicolumn{2}{l|}{20} & \multicolumn{2}{l|}{10} & \multicolumn{2}{l|}{20} & \multicolumn{2}{l|}{10} & \multicolumn{2}{l}{20} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule
GROOV & \multicolumn{1}{l}{33.3} & \multicolumn{1}{l|}{35.7} & \multicolumn{1}{l}{16.8} & \multicolumn{1}{l|}{36.0} & \multicolumn{1}{l}{38.4} & \multicolumn{1}{l|}{20.2} & \multicolumn{1}{l}{19.8} & \multicolumn{1}{l|}{20.9} & \multicolumn{1}{l}{70.3} & \multicolumn{1}{l|}{18.6} & \multicolumn{1}{l}{54.1} & \multicolumn{1}{l}{28.4}\\ 
One2Seq (correct) & \multicolumn{1}{l}{51.3} & \multicolumn{1}{l|}{54.0} & \multicolumn{1}{l}{34.4} & \multicolumn{1}{l|}{71.2} & \multicolumn{1}{l}{70.5} & \multicolumn{1}{l|}{37.5} & \multicolumn{1}{l}{58.5} & \multicolumn{1}{l|}{61.5} & \multicolumn{1}{l}{70.9} & \multicolumn{1}{l|}{19.4} & \multicolumn{1}{l}{79.3} & \multicolumn{1}{l}{43.5}\\ 
% One2Seq (no eos) & \multicolumn{1}{l}{50.2} & \multicolumn{1}{l|}{52.2} & \multicolumn{1}{l}{34.8} & \multicolumn{1}{l|}{72.1} & \multicolumn{1}{l}{68.8} & \multicolumn{1}{l|}{36.6} & \multicolumn{1}{l}{57.8} & \multicolumn{1}{l|}{61.1} & \multicolumn{1}{l}{74.8} & \multicolumn{1}{l|}{20.6} & \multicolumn{1}{l}{81.4} & \multicolumn{1}{l}{44.8}\\ 
One2One & \multicolumn{1}{l}{40.8} & \multicolumn{1}{l|}{41.5} & \multicolumn{1}{l}{29.2} & \multicolumn{1}{l|}{59.6} & \multicolumn{1}{l}{57.4} & \multicolumn{1}{l|}{30.6} & \multicolumn{1}{l}{44.0} & \multicolumn{1}{l|}{46.9} & \multicolumn{1}{l}{43.3} & \multicolumn{1}{l|}{12.0} & \multicolumn{1}{l}{31.9} & \multicolumn{1}{l}{17.7}\\ 
PUSL & \multicolumn{1}{l}{52.2} & \multicolumn{1}{l|}{54.9} & \multicolumn{1}{l}{36.4} & \multicolumn{1}{l|}{75.5} & \multicolumn{1}{l}{71.0} & \multicolumn{1}{l|}{37.7} & \multicolumn{1}{l}{61.5} & \multicolumn{1}{l|}{64.8} & \multicolumn{1}{l}{85.6} & \multicolumn{1}{l|}{23.7} & \multicolumn{1}{l}{86.6} & \multicolumn{1}{l}{47.8}\\ \midrule
& \multicolumn{12}{c}{Our Proprietary data} \\ \midrule
& \multicolumn{4}{l|}{Narrow ($|\mathcal{Y}| \leq 3$)} & \multicolumn{4}{l|}{Medium ($ 4 \leq |\mathcal{Y}| \leq 5$)} & \multicolumn{4}{l}{Diverse ($ 6 \leq |\mathcal{Y}|)$} \\ \midrule
Budget@k & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{5} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{5} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l}{5} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule
GROOV & \multicolumn{1}{l}{16.2} & \multicolumn{1}{l|}{27.1} & \multicolumn{1}{l}{9.7} & \multicolumn{1}{l|}{27.1} & \multicolumn{1}{l}{21.8} & \multicolumn{1}{l|}{14.9} & \multicolumn{1}{l}{13.0} & \multicolumn{1}{l|}{14.9} & \multicolumn{1}{l}{25.5} & \multicolumn{1}{l|}{7.9} & \multicolumn{1}{l}{15.3} & \multicolumn{1}{l}{7.9}\\ 
One2Seq (correct) & \multicolumn{1}{l}{20.8} & \multicolumn{1}{l|}{33.4} & \multicolumn{1}{l}{13.0} & \multicolumn{1}{l|}{34.8} & \multicolumn{1}{l}{31.5} & \multicolumn{1}{l|}{21.6} & \multicolumn{1}{l}{20.2} & \multicolumn{1}{l|}{23.2} & \multicolumn{1}{l}{40.0} & \multicolumn{1}{l|}{12.0} & \multicolumn{1}{l}{26.0} & \multicolumn{1}{l}{13.0}\\ 
% One2Seq (no eos) & \multicolumn{1}{l}{22.0} & \multicolumn{1}{l|}{35.3} & \multicolumn{1}{l}{14.1} & \multicolumn{1}{l|}{37.5} & \multicolumn{1}{l}{33.9} & \multicolumn{1}{l|}{23.2} & \multicolumn{1}{l}{21.9} & \multicolumn{1}{l|}{25.1} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{12.8} & \multicolumn{1}{l}{27.9} & \multicolumn{1}{l}{14.0}\\ 
One2One & \multicolumn{1}{l}{27.1} & \multicolumn{1}{l|}{42.7} & \multicolumn{1}{l}{20.1} & \multicolumn{1}{l|}{51.9} & \multicolumn{1}{l}{43.6} & \multicolumn{1}{l|}{29.9} & \multicolumn{1}{l}{34.7} & \multicolumn{1}{l|}{39.6} & \multicolumn{1}{l}{58.0} & \multicolumn{1}{l|}{17.5} & \multicolumn{1}{l}{49.7} & \multicolumn{1}{l}{24.5}\\ 
PUSL & \multicolumn{1}{l}{27.8} & \multicolumn{1}{l|}{44.1} & \multicolumn{1}{l}{18.0} & \multicolumn{1}{l|}{47.3} & \multicolumn{1}{l}{43.0} & \multicolumn{1}{l|}{29.4} & \multicolumn{1}{l}{28.7} & \multicolumn{1}{l|}{32.7} & \multicolumn{1}{l}{54.2} & \multicolumn{1}{l|}{16.5} & \multicolumn{1}{l}{37.8} & \multicolumn{1}{l}{19.1}\\


\bottomrule
\end{tabular}
% \label{tab:main}
\caption{Evaluation on budget@k. \haoran{I want to use both bold text and cell highlight.}}
\end{table*}



% \begin{table*}[]
% \centering
% \scriptsize
% \begin{tabular}{|l|llllllllllllllllll|}
% \hline
%            & \multicolumn{6}{l|}{Short}                                                                                                                                            & \multicolumn{6}{l|}{Medium}                                                                                                                                           & \multicolumn{6}{l|}{Long}                                                                                                                        \\ \hline
%            & \multicolumn{18}{l|}{AmazonCat}                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
% k          & \multicolumn{3}{l|}{5}                                                            & \multicolumn{3}{l|}{10}                                                           & \multicolumn{3}{l|}{5}                                                            & \multicolumn{3}{l|}{10}                                                           & \multicolumn{3}{l|}{5}                                                            & \multicolumn{3}{l|}{10}                                      \\ \hline
%            & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & \multicolumn{1}{l|}{F}    & \multicolumn{1}{l|}{P}    & \multicolumn{1}{l|}{R}    & F    \\ \hline
% PUSL       & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l|}{42.2} & 42.2 \\ \hline
% DS(o2o)    & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     &      \\ \hline
% GROOV      & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     &      \\ \hline
% DS(catseq) & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     &      \\ \hline
% \end{tabular}
% \end{table*}

==> tables/budgetk_modified_with_K.tex <==
% \setlength{\columnsep}{-2.5cm}
\setlength{\tabcolsep}{4pt}

\begin{table*}[t]
% \label{Table:perf-comparison}
\centering
% \small
\scriptsize
\begin{tabular}{l|llllllllllllllllll}
% \begin{tabular}{l|cccccccccccccccccc}

% \begin{tabular}{l|p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}p{0.035\textwidth}}


\toprule
& \multicolumn{18}{c}{AmazonCat} \\ \midrule
& \multicolumn{6}{l|}{Narrow ($|\mathcal{Y}| \leq 3$) (33.9\%)} & \multicolumn{6}{l|}{Medium ($ 4 \leq |\mathcal{Y}| \leq 9$) (56.3\%)} & \multicolumn{6}{l}{Diverse ($ 10 \leq |\mathcal{Y}|$) (9.6\%)} \\ \midrule
top-$k$ & \multicolumn{3}{l|}{3} & \multicolumn{3}{l|}{6} & \multicolumn{3}{l|}{3} & \multicolumn{3}{l|}{6} & \multicolumn{3}{l|}{3} & \multicolumn{3}{l}{6} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l}{\#K} \\ \midrule
GROOV & \multicolumn{1}{l}{\textbf{50.6}} & \multicolumn{1}{l}{\textbf{78.2}} & \multicolumn{1}{l|}{\high{2.2}} & \multicolumn{1}{l}{\textbf{25.4}} & \multicolumn{1}{l}{\textbf{78.5}} & \multicolumn{1}{l|}{2.3} & \multicolumn{1}{l}{\textbf{79}} & \multicolumn{1}{l}{\textbf{39.1}} & \multicolumn{1}{l|}{\high{2.6}} & \multicolumn{1}{l}{46.6} & \multicolumn{1}{l}{45.8} & \multicolumn{1}{l|}{3.2} & \multicolumn{1}{l}{\textbf{84.8}} & \multicolumn{1}{l}{\textbf{19.6}} & \multicolumn{1}{l|}{\high{2.7}} & \multicolumn{1}{l}{52.8} & \multicolumn{1}{l}{24.3} & \multicolumn{1}{l}{3.5} \\ 
One2Seq & \multicolumn{1}{l}{18.0} & \multicolumn{1}{l}{31.6} & \multicolumn{1}{l|}{\high{2.8}} & \multicolumn{1}{l}{15.4} & \multicolumn{1}{l}{51.3} & \multicolumn{1}{l|}{\high{5.4}} & \multicolumn{1}{l}{54.1} & \multicolumn{1}{l}{25.7} & \multicolumn{1}{l|}{\high{2.9}} & \multicolumn{1}{l}{44.2} & \multicolumn{1}{l}{41.6} & \multicolumn{1}{l|}{\high{5.6}} & \multicolumn{1}{l}{67.8} & \multicolumn{1}{l}{15.5} & \multicolumn{1}{l|}{\high{2.9}} & \multicolumn{1}{l}{61.1} & \multicolumn{1}{l}{27.9} & \multicolumn{1}{l}{\high{5.9}} \\ 
% One2Seq (no eos) & \multicolumn{1}{l}{18.8} & \multicolumn{1}{l|}{33.2} & \multicolumn{1}{l}{16.8} & \multicolumn{1}{l|}{54.6} & \multicolumn{1}{l}{63.0} & \multicolumn{1}{l|}{29.9} & \multicolumn{1}{l}{52.0} & \multicolumn{1}{l|}{48.9} & \multicolumn{1}{l}{78.6} & \multicolumn{1}{l|}{18.1} & \multicolumn{1}{l}{70.5} & \multicolumn{1}{l}{32.3}\\ 
One2One & \multicolumn{1}{l}{24.4} & \multicolumn{1}{l}{34.5} & \multicolumn{1}{l|}{\high{3.0}} & \multicolumn{1}{l}{19.7} & \multicolumn{1}{l}{57.5} & \multicolumn{1}{l|}{\high{6.0}} & \multicolumn{1}{l}{67.6} & \multicolumn{1}{l}{32.8} & \multicolumn{1}{l|}{\high{3.0}} & \multicolumn{1}{l}{\textbf{56.9}} & \multicolumn{1}{l}{\textbf{54.8}} & \multicolumn{1}{l|}{\high{6.0}} & \multicolumn{1}{l}{78.5} & \multicolumn{1}{l}{18.0} & \multicolumn{1}{l|}{\high{3.0}} & \multicolumn{1}{l}{69.3} & \multicolumn{1}{l}{31.8} & \multicolumn{1}{l}{\high{6.0}} \\ 
PUSL & \multicolumn{1}{l}{21.7} & \multicolumn{1}{l}{37.6} & \multicolumn{1}{l|}{\high{2.9}} & \multicolumn{1}{l}{20} & \multicolumn{1}{l}{63.7} & \multicolumn{1}{l|}{\high{5.8}} & \multicolumn{1}{l}{64.6} & \multicolumn{1}{l}{30.7} & \multicolumn{1}{l|}{\high{2.9}} & \multicolumn{1}{l}{55.4} & \multicolumn{1}{l}{52.5} & \multicolumn{1}{l|}{\high{5.8}} & \multicolumn{1}{l}{79.1} & \multicolumn{1}{l}{18.2} & \multicolumn{1}{l|}{\high{3.0}} & \multicolumn{1}{l}{\textbf{71.5}} & \multicolumn{1}{l}{\textbf{32.7}} & \multicolumn{1}{l}{\high{5.9}} \\ \midrule

& \multicolumn{18}{c}{Wikipedia-1M} \\ \midrule
& \multicolumn{6}{l|}{Narrow ($|\mathcal{Y}| \leq 4$) (60.0\%)} & \multicolumn{6}{l|}{Medium ($ 5 \leq |\mathcal{Y}| \leq 10$) (31.0\%)} & \multicolumn{6}{l}{Diverse ($ 11 \leq |\mathcal{Y}|$) (9.0\%) } \\ \midrule
top-$k$ & \multicolumn{3}{l|}{2} & \multicolumn{3}{l|}{4} & \multicolumn{3}{l|}{2} & \multicolumn{3}{l|}{4} & \multicolumn{3}{l|}{2} & \multicolumn{3}{l}{4} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l}{\#K} \\ \midrule
GROOV & \multicolumn{1}{l}{\textbf{51.6}} & \multicolumn{1}{l}{\textbf{48.3}} & \multicolumn{1}{l|}{\high{1.6}} & \multicolumn{1}{l}{28.5} & \multicolumn{1}{l}{\textbf{51.6}} & \multicolumn{1}{l|}{1.9} & \multicolumn{1}{l}{\textbf{79.1}} & \multicolumn{1}{l}{\textbf{25.7}} & \multicolumn{1}{l|}{\high{1.9}} & \multicolumn{1}{l}{\textbf{56.7}} & \multicolumn{1}{l}{\textbf{36.1}} & \multicolumn{1}{l|}{2.9} & \multicolumn{1}{l}{\textbf{92.1}} & \multicolumn{1}{l}{\textbf{13.8}} & \multicolumn{1}{l|}{\high{1.9}} & \multicolumn{1}{l}{\textbf{77.6}} & \multicolumn{1}{l}{\textbf{23.0}} & \multicolumn{1}{l}{\high{3.5}} \\ 
One2Seq & \multicolumn{1}{l}{19.6} & \multicolumn{1}{l}{15.5} & \multicolumn{1}{l|}{1.8} & \multicolumn{1}{l}{12.2} & \multicolumn{1}{l}{19.3} & \multicolumn{1}{l|}{3.1} & \multicolumn{1}{l}{54.8} & \multicolumn{1}{l}{16.5} & \multicolumn{1}{l|}{1.9} & \multicolumn{1}{l}{36.3} & \multicolumn{1}{l}{21.7} & \multicolumn{1}{l|}{3.6} & \multicolumn{1}{l}{75.7} & \multicolumn{1}{l}{10.6} & \multicolumn{1}{l|}{1.9} & \multicolumn{1}{l}{58.0} & \multicolumn{1}{l}{16.1} & \multicolumn{1}{l}{3.8} \\ 
% One2Seq (no eos) & \multicolumn{1}{l}{20.6} & \multicolumn{1}{l|}{16.3} & \multicolumn{1}{l}{13.1} & \multicolumn{1}{l|}{20.9} & \multicolumn{1}{l}{55.9} & \multicolumn{1}{l|}{16.8} & \multicolumn{1}{l}{37.5} & \multicolumn{1}{l|}{22.4} & \multicolumn{1}{l}{77.0} & \multicolumn{1}{l|}{10.8} & \multicolumn{1}{l}{59.8} & \multicolumn{1}{l}{16.6}\\ 
One2One & \multicolumn{1}{l}{40.3} & \multicolumn{1}{l}{36.4} & \multicolumn{1}{l|}{\high{2.0}} & \multicolumn{1}{l}{\textbf{29.0}} & \multicolumn{1}{l}{50.5} & \multicolumn{1}{l|}{\high{3.9}} & \multicolumn{1}{l}{62.5} & \multicolumn{1}{l}{19.2} & \multicolumn{1}{l|}{\high{2.0}} & \multicolumn{1}{l}{53.1} & \multicolumn{1}{l}{32.6} & \multicolumn{1}{l|}{\high{4.0}} & \multicolumn{1}{l}{75.0} & \multicolumn{1}{l}{10.5} & \multicolumn{1}{l|}{\high{2.0}} & \multicolumn{1}{l}{68.5} & \multicolumn{1}{l}{19.1} & \multicolumn{1}{l}{\high{4.0}} \\ 
PUSL & \multicolumn{1}{l}{17.3} & \multicolumn{1}{l}{13.3} & \multicolumn{1}{l|}{\high{1.8}} & \multicolumn{1}{l}{11.1} & \multicolumn{1}{l}{17.1} & \multicolumn{1}{l|}{\high{3.1}} & \multicolumn{1}{l}{53.3} & \multicolumn{1}{l}{16.0} & \multicolumn{1}{l|}{\high{1.9}} & \multicolumn{1}{l}{35.3} & \multicolumn{1}{l}{21.1} & \multicolumn{1}{l|}{\high{3.5}} & \multicolumn{1}{l}{74.8} & \multicolumn{1}{l}{10.5} & \multicolumn{1}{l|}{\high{1.9}} & \multicolumn{1}{l}{57.1} & \multicolumn{1}{l}{15.8} & \multicolumn{1}{l}{\high{3.7}} \\ \midrule

& \multicolumn{18}{c}{EURLex4.3k} \\ \midrule
& \multicolumn{6}{l|}{Narrow ($|\mathcal{Y}| \leq 14$) (51.9\%)} & \multicolumn{6}{l|}{Medium ($ 15 \leq |\mathcal{Y}| \leq 28$) (38.7\%)} & \multicolumn{6}{l}{Diverse ($ 29 \leq |\mathcal{Y}|$) (9.2\%)} \\ \midrule
top-$k$ & \multicolumn{3}{l|}{10} & \multicolumn{3}{l|}{20} & \multicolumn{3}{l|}{10} & \multicolumn{3}{l|}{20} & \multicolumn{3}{l|}{10} & \multicolumn{3}{l}{20} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l}{\#K} \\ \midrule
GROOV & \multicolumn{1}{l}{33.3} & \multicolumn{1}{l}{35.7} & \multicolumn{1}{l|}{6.3} & \multicolumn{1}{l}{16.8} & \multicolumn{1}{l}{36.0} & \multicolumn{1}{l|}{6.7} & \multicolumn{1}{l}{38.4} & \multicolumn{1}{l}{20.2} & \multicolumn{1}{l|}{7.4} & \multicolumn{1}{l}{19.8} & \multicolumn{1}{l}{20.9} & \multicolumn{1}{l|}{8.4} & \multicolumn{1}{l}{70.3} & \multicolumn{1}{l}{18.6} & \multicolumn{1}{l|}{\high{9.3}} & \multicolumn{1}{l}{54.1} & \multicolumn{1}{l}{28.4} & \multicolumn{1}{l}{15.1} \\ 
One2Seq & \multicolumn{1}{l}{51.3} & \multicolumn{1}{l}{54.0} & \multicolumn{1}{l|}{\high{9.6}} & \multicolumn{1}{l}{34.4} & \multicolumn{1}{l}{71.2} & \multicolumn{1}{l|}{17.2} & \multicolumn{1}{l}{70.5} & \multicolumn{1}{l}{37.5} & \multicolumn{1}{l|}{\high{9.8}} & \multicolumn{1}{l}{58.5} & \multicolumn{1}{l}{61.5} & \multicolumn{1}{l|}{18.4} & \multicolumn{1}{l}{70.9} & \multicolumn{1}{l}{19.4} & \multicolumn{1}{l|}{\high{9.9}} & \multicolumn{1}{l}{79.3} & \multicolumn{1}{l}{43.5} & \multicolumn{1}{l}{\high{19.6}} \\ 
% One2Seq (no eos) & \multicolumn{1}{l}{50.2} & \multicolumn{1}{l|}{52.2} & \multicolumn{1}{l}{34.8} & \multicolumn{1}{l|}{72.1} & \multicolumn{1}{l}{68.8} & \multicolumn{1}{l|}{36.6} & \multicolumn{1}{l}{57.8} & \multicolumn{1}{l|}{61.1} & \multicolumn{1}{l}{74.8} & \multicolumn{1}{l|}{20.6} & \multicolumn{1}{l}{81.4} & \multicolumn{1}{l}{44.8}\\ 
One2One & \multicolumn{1}{l}{40.8} & \multicolumn{1}{l}{41.5} & \multicolumn{1}{l|}{\high{10.0}} & \multicolumn{1}{l}{29.2} & \multicolumn{1}{l}{59.6} & \multicolumn{1}{l|}{\high{20.0}} & \multicolumn{1}{l}{57.4} & \multicolumn{1}{l}{30.6} & \multicolumn{1}{l|}{\high{10.0}} & \multicolumn{1}{l}{44.0} & \multicolumn{1}{l}{46.9} & \multicolumn{1}{l|}{\high{20.0}} & \multicolumn{1}{l}{43.3} & \multicolumn{1}{l}{12.0} & \multicolumn{1}{l|}{\high{10.0}} & \multicolumn{1}{l}{31.9} & \multicolumn{1}{l}{17.7} & \multicolumn{1}{l}{\high{20.0}}\\ 
PUSL & \multicolumn{1}{l}{\textbf{52.2}} & \multicolumn{1}{l}{\textbf{54.9}} &  \multicolumn{1}{l|}{\high{9.8}} & \multicolumn{1}{l}{\textbf{36.4}} & \multicolumn{1}{l}{\textbf{75.5}} & \multicolumn{1}{l|}{17.9} & \multicolumn{1}{l}{\textbf{71.0}} & \multicolumn{1}{l}{\textbf{37.7}} & \multicolumn{1}{l|}{\high{9.9}} & \multicolumn{1}{l}{\textbf{61.5}} & \multicolumn{1}{l}{\textbf{64.8}} & \multicolumn{1}{l|}{\high{19.0}} & \multicolumn{1}{l}{\textbf{85.6}} & \multicolumn{1}{l}{\textbf{23.7}} & \multicolumn{1}{l|}{\high{9.9}} & \multicolumn{1}{l}{\textbf{86.6}} & \multicolumn{1}{l}{\textbf{47.8}} & \multicolumn{1}{l}{\high{19.8}} \\ \midrule

& \multicolumn{18}{c}{Our Proprietary Data} \\ \midrule
& \multicolumn{6}{l|}{Narrow ($|\mathcal{Y}| \leq 3$) (81.3\%)} & \multicolumn{6}{l|}{Medium ($ 4 \leq |\mathcal{Y}| \leq 5$) (7.9\%)} & \multicolumn{6}{l}{Diverse ($ 6 \leq |\mathcal{Y}|)$ (10.6\%)} \\ \midrule
top-$k$ & \multicolumn{3}{l|}{3} & \multicolumn{3}{l|}{5} & \multicolumn{3}{l|}{3} & \multicolumn{3}{l|}{5} & \multicolumn{3}{l|}{3} & \multicolumn{3}{l}{5} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l|}{\#K} & \multicolumn{1}{l}{P} & \multicolumn{1}{l}{R} & \multicolumn{1}{l}{\#K} \\ \midrule
GROOV & \multicolumn{1}{l}{16.2} & \multicolumn{1}{l}{27.1} & \multicolumn{1}{l|}{1.0} & \multicolumn{1}{l}{9.7} & \multicolumn{1}{l}{27.1} & \multicolumn{1}{l|}{1.0} & \multicolumn{1}{l}{21.8} & \multicolumn{1}{l}{14.9} & \multicolumn{1}{l|}{1.0} & \multicolumn{1}{l}{13.0} & \multicolumn{1}{l}{14.9} & \multicolumn{1}{l|}{1.0} & \multicolumn{1}{l}{25.5} & \multicolumn{1}{l}{7.9} & \multicolumn{1}{l|}{1.0} & \multicolumn{1}{l}{15.3} & \multicolumn{1}{l}{7.9} & \multicolumn{1}{l}{1.0} \\ 
One2Seq & \multicolumn{1}{l}{20.8} & \multicolumn{1}{l}{33.4} & \multicolumn{1}{l|}{1.8} & \multicolumn{1}{l}{13.0} & \multicolumn{1}{l}{34.8} & \multicolumn{1}{l|}{2.1} & \multicolumn{1}{l}{31.5} & \multicolumn{1}{l}{21.6} & \multicolumn{1}{l|}{1.9} & \multicolumn{1}{l}{20.2} & \multicolumn{1}{l}{23.2} & \multicolumn{1}{l|}{2.1} & \multicolumn{1}{l}{40.0} & \multicolumn{1}{l}{12.0} & \multicolumn{1}{l|}{1.8} & \multicolumn{1}{l}{26.0} & \multicolumn{1}{l}{13.0} & \multicolumn{1}{l}{2.0} \\ 
% One2Seq (no eos) & \multicolumn{1}{l}{22.0} & \multicolumn{1}{l|}{35.3} & \multicolumn{1}{l}{14.1} & \multicolumn{1}{l|}{37.5} & \multicolumn{1}{l}{33.9} & \multicolumn{1}{l|}{23.2} & \multicolumn{1}{l}{21.9} & \multicolumn{1}{l|}{25.1} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{12.8} & \multicolumn{1}{l}{27.9} & \multicolumn{1}{l}{14.0}\\ 
One2One & \multicolumn{1}{l}{27.1} & \multicolumn{1}{l}{42.7} & \multicolumn{1}{l|}{\high{3.0}} & \multicolumn{1}{l}{\textbf{20.1}} & \multicolumn{1}{l}{\textbf{51.9}} & \multicolumn{1}{l|}{\high{4.9}} & \multicolumn{1}{l}{\textbf{43.6}} & \multicolumn{1}{l}{\textbf{29.9}} & \multicolumn{1}{l|}{\high{3.0}} & \multicolumn{1}{l}{\textbf{34.7}} & \multicolumn{1}{l}{\textbf{39.6}} & \multicolumn{1}{l|}{\high{5.0}} & \multicolumn{1}{l}{\textbf{58.0}} & \multicolumn{1}{l}{\textbf{17.5}} & \multicolumn{1}{l|}{\high{3.0}} & \multicolumn{1}{l}{\textbf{49.7}} & \multicolumn{1}{l}{\textbf{24.5}} & \multicolumn{1}{l}{\high{5.0}} \\ 
PUSL & \multicolumn{1}{l}{\textbf{27.8}} & \multicolumn{1}{l}{\textbf{44.1}} & \multicolumn{1}{l|}{\high{2.4}} & \multicolumn{1}{l}{18.0} & \multicolumn{1}{l}{47.3} & \multicolumn{1}{l|}{3.1} & \multicolumn{1}{l}{43.0} & \multicolumn{1}{l}{29.4} & \multicolumn{1}{l|}{\high{2.4}} & \multicolumn{1}{l}{28.7} & \multicolumn{1}{l}{32.7} & \multicolumn{1}{l|}{3.0} & \multicolumn{1}{l}{54.2} & \multicolumn{1}{l}{16.5} & \multicolumn{1}{l|}{\high{2.4}} & \multicolumn{1}{l}{37.8} & \multicolumn{1}{l}{19.1} & \multicolumn{1}{l}{3.0} \\


\bottomrule
\end{tabular}
\caption{Evaluation on test sets under different ground truth diversity. We report the precision (P), recall (R) and average number of the generated keyphrase (\#K) for different top-$k$ requirement. Bold text are the highest score. Highlight cells are the generated keyphrases roughly satisfies the required k, misses less than 1 average predicted keyphrase. Narrow ($|\mathcal{Y}| \leq 3$) (81.3\%) means each data points in narrow test set only have less than 3 keyphrase, and they cover 81.3\% of the corpus.
\haoran{tagging vs categorization}
% \rui{move this table earlier in page 6.}
}
\label{tab:gtdependent}
\end{table*}

==> tables/budgetk_noeos.tex <==
\begin{table*}[t]
% \label{Table:perf-comparison}
\centering
% \small
\scriptsize
\begin{tabular}{l|llllllllllll}
\toprule
& \multicolumn{12}{c}{AmazonCat} \\ \midrule
& \multicolumn{4}{l|}{Short ($|\mathcal{Y}| \leq 3$)} & \multicolumn{4}{l|}{Medium ($ 4 \leq |\mathcal{Y}| \leq 9$)} & \multicolumn{4}{l}{Long ($ 10 \leq |\mathcal{Y}|$)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{6} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{6} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l}{6} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule

One2Seq (correct) & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l}-\\ 
One2Seq (no eos) & \multicolumn{1}{l}{18.8} & \multicolumn{1}{l|}{33.2} & \multicolumn{1}{l}{16.8} & \multicolumn{1}{l|}{54.6} & \multicolumn{1}{l}{63.0} & \multicolumn{1}{l|}{29.9} & \multicolumn{1}{l}{52.0} & \multicolumn{1}{l|}{48.9} & \multicolumn{1}{l}{78.6} & \multicolumn{1}{l|}{18.1} & \multicolumn{1}{l}{70.5} & \multicolumn{1}{l}{32.3}\\ 



PUSL & \multicolumn{1}{l}{21.7} & \multicolumn{1}{l|}{37.6} & \multicolumn{1}{l}{20} & \multicolumn{1}{l|}{63.7} & \multicolumn{1}{l}{64.6} & \multicolumn{1}{l|}{30.7} & \multicolumn{1}{l}{55.4} & \multicolumn{1}{l|}{52.5} & \multicolumn{1}{l}{79.1} & \multicolumn{1}{l|}{18.2} & \multicolumn{1}{l}{71.5} & \multicolumn{1}{l}{32.7}\\ \midrule
& \multicolumn{12}{c}{Wikipedia-1M} \\ \midrule
& \multicolumn{4}{l|}{Short ($|\mathcal{Y}| \leq 4$)} & \multicolumn{4}{l|}{Medium ($ 5 \leq |\mathcal{Y}| \leq 10$)} & \multicolumn{4}{l}{Long ($ 11 \leq |\mathcal{Y}|$)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{2} & \multicolumn{2}{l|}{4} & \multicolumn{2}{l|}{2} & \multicolumn{2}{l|}{4} & \multicolumn{2}{l|}{2} & \multicolumn{2}{l}{4} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule

One2Seq (correct) & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{42.2} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l}{42.2}\\ 
One2Seq (no eos) & \multicolumn{1}{l}{20.6} & \multicolumn{1}{l|}{16.3} & \multicolumn{1}{l}{13.1} & \multicolumn{1}{l|}{20.9} & \multicolumn{1}{l}{55.9} & \multicolumn{1}{l|}{16.8} & \multicolumn{1}{l}{37.5} & \multicolumn{1}{l|}{22.4} & \multicolumn{1}{l}{77.0} & \multicolumn{1}{l|}{10.8} & \multicolumn{1}{l}{59.8} & \multicolumn{1}{l}{16.6}\\ 

PUSL & \multicolumn{1}{l}{17.3} & \multicolumn{1}{l|}{13.3} & \multicolumn{1}{l}{11.1} & \multicolumn{1}{l|}{17.1} & \multicolumn{1}{l}{53.3} & \multicolumn{1}{l|}{16.0} & \multicolumn{1}{l}{35.3} & \multicolumn{1}{l|}{21.1} & \multicolumn{1}{l}{74.8} & \multicolumn{1}{l|}{10.5} & \multicolumn{1}{l}{57.1} & \multicolumn{1}{l}{15.8}\\ \midrule
& \multicolumn{12}{c}{EURLex4.3k} \\ \midrule
& \multicolumn{4}{l|}{Short ($|\mathcal{Y}| \leq 14$)} & \multicolumn{4}{l|}{Medium ($ 15 \leq |\mathcal{Y}| \leq 28$)} & \multicolumn{4}{l}{Long ($ 29 \leq |\mathcal{Y}|$)} \\ \midrule
Budget@k & \multicolumn{2}{l|}{10} & \multicolumn{2}{l|}{20} & \multicolumn{2}{l|}{10} & \multicolumn{2}{l|}{20} & \multicolumn{2}{l|}{10} & \multicolumn{2}{l}{20} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule

One2Seq (correct) & \multicolumn{1}{l}{51.3} & \multicolumn{1}{l|}{54.0} & \multicolumn{1}{l}{34.4} & \multicolumn{1}{l|}{71.2} & \multicolumn{1}{l}{70.5} & \multicolumn{1}{l|}{37.5} & \multicolumn{1}{l}{58.5} & \multicolumn{1}{l|}{61.5} & \multicolumn{1}{l}{70.9} & \multicolumn{1}{l|}{19.4} & \multicolumn{1}{l}{79.3} & \multicolumn{1}{l}{43.5}\\ 
One2Seq (no eos) & \multicolumn{1}{l}{50.2} & \multicolumn{1}{l|}{52.2} & \multicolumn{1}{l}{34.8} & \multicolumn{1}{l|}{72.1} & \multicolumn{1}{l}{68.8} & \multicolumn{1}{l|}{36.6} & \multicolumn{1}{l}{57.8} & \multicolumn{1}{l|}{61.1} & \multicolumn{1}{l}{74.8} & \multicolumn{1}{l|}{20.6} & \multicolumn{1}{l}{81.4} & \multicolumn{1}{l}{44.8}\\ 

PUSL & \multicolumn{1}{l}{52.2} & \multicolumn{1}{l|}{54.9} & \multicolumn{1}{l}{36.4} & \multicolumn{1}{l|}{75.5} & \multicolumn{1}{l}{71.0} & \multicolumn{1}{l|}{37.7} & \multicolumn{1}{l}{61.5} & \multicolumn{1}{l|}{64.8} & \multicolumn{1}{l}{85.6} & \multicolumn{1}{l|}{23.7} & \multicolumn{1}{l}{86.6} & \multicolumn{1}{l}{47.8}\\ \midrule
& \multicolumn{12}{c}{Our Proprietary data} \\ \midrule
& \multicolumn{4}{l|}{Short ($|\mathcal{Y}| \leq 3$)} & \multicolumn{4}{l|}{Medium ($ 4 \leq |\mathcal{Y}| \leq 5$)} & \multicolumn{4}{l}{Long ($ 6 \leq |\mathcal{Y}|)$} \\ \midrule
Budget@k & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{5} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{5} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l}{5} \\ 
& \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l|}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & \multicolumn{1}{l|}{R} & \multicolumn{1}{l}{P} & R \\ \midrule

One2Seq (correct) & \multicolumn{1}{l}{20.8} & \multicolumn{1}{l|}{33.4} & \multicolumn{1}{l}{13.0} & \multicolumn{1}{l|}{34.8} & \multicolumn{1}{l}{31.5} & \multicolumn{1}{l|}{21.6} & \multicolumn{1}{l}{20.2} & \multicolumn{1}{l|}{23.2} & \multicolumn{1}{l}{40.0} & \multicolumn{1}{l|}{12.0} & \multicolumn{1}{l}{26.0} & \multicolumn{1}{l}{13.0}\\ 
One2Seq (no eos) & \multicolumn{1}{l}{22.0} & \multicolumn{1}{l|}{35.3} & \multicolumn{1}{l}{14.1} & \multicolumn{1}{l|}{37.5} & \multicolumn{1}{l}{33.9} & \multicolumn{1}{l|}{23.2} & \multicolumn{1}{l}{21.9} & \multicolumn{1}{l|}{25.1} & \multicolumn{1}{l}{42.2} & \multicolumn{1}{l|}{12.8} & \multicolumn{1}{l}{27.9} & \multicolumn{1}{l}{14.0}\\ 
PUSL & \multicolumn{1}{l}{27.8} & \multicolumn{1}{l|}{44.1} & \multicolumn{1}{l}{18.0} & \multicolumn{1}{l|}{47.3} & \multicolumn{1}{l}{43.0} & \multicolumn{1}{l|}{29.4} & \multicolumn{1}{l}{28.7} & \multicolumn{1}{l|}{32.7} & \multicolumn{1}{l}{54.2} & \multicolumn{1}{l|}{16.5} & \multicolumn{1}{l}{37.8} & \multicolumn{1}{l}{19.1}\\


\bottomrule
\end{tabular}
\label{tab:noeos}
\caption{catseq no eos vs pusl}
\end{table*}



==> tables/ebay_hot_vs_rare.tex <==
\begin{table*}[h]
\begin{center}
\small
\begin{tabular}{|l|rrrrr|rrrr|rrr|}
\hline
\multirow{2}{*}{} & \multicolumn{5}{c|}{Hot diverse}                                                                                                                        & \multicolumn{4}{c|}{Hot narrow}                                                                                           & \multicolumn{3}{c|}{Rare narrow}  \\ \cline{2-13} 
                  & \multicolumn{1}{l|}{G} & \multicolumn{1}{l|}{U}   & \multicolumn{1}{l|}{Rel} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{l|}{G} & \multicolumn{1}{l|}{U}   & \multicolumn{1}{l|}{Rel} & \multicolumn{1}{c|}{R} & \multicolumn{1}{l|}{G} & \multicolumn{1}{l|}{U}   & \multicolumn{1}{l|}{Rel} \\ \hline \hline
%GROOV             & \multicolumn{1}{r|}{\textbf{99.1}} & \multicolumn{1}{r|}{94.5} & \multicolumn{1}{r|}{\textbf{91.8}}     & \multicolumn{1}{r|}{18.0}    & 3.2                       & \multicolumn{1}{r|}{99.0} & \multicolumn{1}{r|}{90.3} & \multicolumn{1}{r|}{89.3}     & 4.1                          & \multicolumn{1}{r|}{95.1} & \multicolumn{1}{r|}{77.2} & 76.2         \\
%catseq            & \multicolumn{1}{r|}{95.8} & \multicolumn{1}{r|}{\textbf{95.8}} & \multicolumn{1}{r|}{91.6}     & \multicolumn{1}{r|}{32.4}    & 5.9                       & \multicolumn{1}{r|}{96.3} & \multicolumn{1}{r|}{83.1} & \multicolumn{1}{r|}{78.8}     & 55.5                         & \multicolumn{1}{r|}{98.0} & \multicolumn{1}{r|}{81.2} & 77.8         
%\\
One2One            & \multicolumn{1}{r|}{92.2}  & \multicolumn{1}{r|}{90.4} & \multicolumn{1}{r|}{84.0}       & \multicolumn{1}{r|}{\textbf{46.3}}      & \textbf{8.5}                        & \multicolumn{1}{r|}{90.4}  & \multicolumn{1}{r|}{61.2} & \multicolumn{1}{r|}{57.8}       & 53.1                            & \multicolumn{1}{r|}{93.0}  & \multicolumn{1}{r|}{61.4} & 57.8                            \\ 
PUSL              & \multicolumn{1}{r|}{90.9}  & \multicolumn{1}{r|}{93.9} & \multicolumn{1}{r|}{\textbf{85.9}}       & \multicolumn{1}{r|}{42.4}      & 8.4                        & \multicolumn{1}{r|}{92.9}  & \multicolumn{1}{r|}{80.1} & \multicolumn{1}{r|}{\textbf{76.5}}       & \textbf{69.3}                           & \multicolumn{1}{r|}{93.7}  & \multicolumn{1}{r|}{\textbf{75.6}} & \textbf{72.3}  
\\ \hline
\end{tabular}
\end{center}
\caption{Ground-truth-free evaluation on top-$5$ generation. G is calculated from GPT-4 based judgement as a substitute for human judgement for textual relevance. U is whether the prediction belongs in the universe of labels. Rel is the advertisement relevance score. P (Precision) and R (Recall). 
% Hot-short: customers think alike in these hot items, and they just cannot come up with other keyphrase, so we only calculate if the budget@k prediction can recall the ground truth. Rare-short: there are not enough keyphrases collected in the database because of fewer click counts, then we can only calculate relevance score.\haoran{hot diverse contains more "majority labels"}
\rui{Pleae unify table styles. I would suggest booktabs}
\rui{move this table earlier in page 7.}
}
\label{tab:gtfree}
\end{table*}



==> tables/ebay_hot_vs_rare_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\small
\centering
\begin{tabular}{@{}l|ccccc|cccc|ccc@{}}
\toprule
                   & \multicolumn{5}{c|}{Hot diverse (0.16\%)}                                                                                                                                                                                                                                       & \multicolumn{4}{c|}{Hot narrow (4.72\%)}                                                                                                                                                                                        & \multicolumn{3}{c}{Rare narrow (95.12\%)}                                                                                                                               \\ \cmidrule(l){2-13} 
\multirow{-2}{*}{} & \multicolumn{1}{c}{P}                                        & \multicolumn{1}{c}{R}                                       & \multicolumn{1}{l}{G} & \multicolumn{1}{l}{U}                                        & \multicolumn{1}{l|}{Rel}                           & \multicolumn{1}{c}{R}                          & \multicolumn{1}{l}{G}                               & \multicolumn{1}{l}{U}                               & \multicolumn{1}{l|}{Rel}                             & \multicolumn{1}{l}{G}                             & \multicolumn{1}{l}{U}                               & \multicolumn{1}{l}{Rel}                             \\ \midrule
OneOne             &  \textbf{46.3} &  \textbf{8.5} & \textbf{92.2}         & \textbf{90.4} & 84.0 & 53.1 & 90.4 &  61.2 &  57.8 & 93 & 61.4 & 57.8 \\ \midrule
PUSL               & 42.4                                                         & 8.4                                                         & 90.9                  & \textbf{93.9}                                                & \textbf{85.9}                                     & \textbf{69.3}                                       & \textbf{92.9}                                       & \textbf{80.1}                                       & \textbf{76.5}                                       & \textbf{93.7}                                     & \textbf{75.6}                                       & \textbf{72.3}                                       \\ \midrule
%GROOV              & 18.0\%                                                       & 3.2\%                                                       & 99.1\%                & 94.5\%                                                       & 91.8\%                                            & 4.1\%                                               & 99.0\%                                              & 90.3\%                                              & 89.3\%                                              & 95.05\%                                           & 77.23\%                                             & 76.24\%                                             \\ \midrule
%catseq             & 32.4\%                                                       & 5.9\%                                                       & 95.8\%                & 95.8\%                                                       & 91.6\%                                            & 55.5\%                                              & 96.3\%                                              & 83.1\%                                              & 78.8\%                                              & 97.96\%                                           & 81.22\%                                             & 77.76\%                                             \\ \bottomrule
\end{tabular}
\caption{Ground-truth-free evaluation on top-$5$ generation. G is the average proportion of key-phrases that are calculated from GPT-4 based judgement as a substitute for human judgement for textual relevance. U is the average proportion of key-phrases that belongs to the universe of labels. Rel is the average advertisement relevance score. P (Precision) and R (Recall). 
% Hot-short: customers think alike in these hot items, and they just cannot come up with other keyphrase, so we only calculate if the budget@k prediction can recall the ground truth. Rare-short: there are not enough keyphrases collected in the database because of fewer click counts, then we can only calculate relevance score.\haoran{hot diverse contains more "majority labels"
\soumik{ground-truth free how? We still have P \& R scores. Should be out of time eval.}
}
\label{tab:gtfree}
\end{table*}

==> tables/general_evaluation.tex <==
\begin{table*}[t]
\centering
\small
    \begin{tabular}{lccc|ccc}
    % {l{5.7cm}c{1.1cm}c{1.1cm}c{1.1cm}|c{1.1cm}c{1.1cm}c{1.1cm}}
     \toprule
     \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{c|}{\textbf{EUR-Lex 4.3K}} & \multicolumn{3}{|c}{\textbf{Wikipedia-1M}} \\
     \cmidrule{2-4} \cmidrule{5-7}
      & \textbf{PSP@1} & \textbf{PSP@3} & \textbf{PSP@5} & \textbf{PSP@1} & \textbf{PSP@3} & \textbf{PSP@5} \\
     \midrule \midrule
     

     ZestXML-tuned~\cite{gupta2021generalized} & 48.01 & 60.29 & 66.15  & \textbf{14.43} & \textbf{15.80} & \textbf{17.31}\\
     AttentionXML~\cite{attentionxml}  & 53.92 & \textbf{63.59} & \textbf{67.85}  & 3.82 & 4.54 & 5.20 \\
     XReg~\cite{xreg} & \textbf{58.06} & 62.99 & 65.97 & 3.48 & 3.51 & 3.83 \\
     Parabel~\cite{parabel} & 46.82 & 58.8 & 64.29 & 2.99 & 3.32 & 3.65 \\ 
     DiSMEC~\cite{BabSch17} & 47.26 &  59.82 & 65.55 & 2.35 & 2.99 & 3.48 \\
     Bonsai~\cite{Bonsai} & 46.41 & 58.83 & 64.44 & 3.19 & 3.61& 4.05 \\
     PfastreXML~\cite{pfast} & 55.30 & 58.00 & 59.91&  2.97 & 2.90 & 3.10 \\
     
     \midrule
     
     FastText ANNS~\cite{fasttext}  & 17.10 & 15.74 & 16.13 & 7.16 & 6.01 & 6.19 \\
     BERT ANNS~\cite{bert-anns} & 4.64 & 3.66 & 3.57 & 10.34 & 8.17 & 8.20 \\
     \midrule
     GROOV & 52.6 & \textbf{63.6} & 67.2 & 9.8 & 13.4 & 15.8 \\
     CatSeq & 52.6 & \textbf{63.6} & 67.2 & 9.8 & 13.4 & 15.8 \\
     One2One & 52.6 & \textbf{63.6} & 67.2 & 9.8 & 13.4 & 15.8 \\
     PUSL & 52.6 & \textbf{63.6} & 67.2 & 9.8 & 13.4 & 15.8 \\
     \midrule


     \bottomrule
    \end{tabular}
    
\caption{\label{psp_table} General evaluation on EUR-Lex 4.3k and Wiki-1m}
\end{table*}

==> tables/gini.tex <==
\begin{table}[t!]
\centering
\scriptsize
\begin{tabular}{l|ll|ll}
\toprule
           & \multicolumn{2}{c|}{Gini} & \multicolumn{2}{c}{GDP} \\ \midrule
           & Groundtruth     & +PUSL    & Groundtruth    & +PUSL   \\
AmazanCat  &          33.7&               &         5.06 &               \\
Wiki-1M    &          41.9&                &     4.90    &               \\
EURLex4.3k &          28.8&                &     15.94    &               \\
Our data   &          31.1&                &       3.09   &              \\ \bottomrule
\end{tabular}
\caption{use PUSL for ground truth kp augmentation \haoran{gdp is an estimated \#K per item. For groundtruth, we reuse the score from table 1.}}
\end{table}

==> tables/model_example.tex <==
\definecolor{ObservedColor}{rgb}{0,0,0} % Black color for observed keyphrases
\definecolor{UnobservedColor}{rgb}{0.5,0.5,0.5} % Grey color for unobserved keyphrases

\begin{table*}[!htbp]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Training Stage} & \textbf{Keyphrases} \\
\hline
Initial & \textcolor{ObservedColor}{$<bok>$MaxMara$<eok>$} \textcolor{UnobservedColor}{$<bok>$wool coat$<eok>$$<bok>$trench coat$<eok>$$<bok>$stylish coat$<eok>$} \\
\hline
Intermediate & \textcolor{ObservedColor}{$<bok>$wool blend$<eok>$$<bok>$designer coat$<eok>$} \textcolor{UnobservedColor}{$<bok>$winter attire$<eok>$$<bok>$high-end outerwear$<eok>$} \\
\hline
Advanced & \textcolor{ObservedColor}{$<bok>$camel coat$<eok>$$<bok>$luxury trench$<eok>$$<bok>$alpaca blend$<eok>$} \textcolor{UnobservedColor}{$<bok>$chic apparel$<eok>$} \\
\hline
\end{tabular}
\caption{Progressive training stages of the model with observed and unobserved keyphrases.}
\label{tab:training_progress}
\end{table*}

==> tables/new_main_table.tex <==
% \setlength{\columnsep}{-2.5cm}
\setlength{\tabcolsep}{4pt}
\begin{table*}[!t]
\centering
\scriptsize
% \begin{tabular}{@{}rrrrrrrrrrrrrrr@{}}
\begin{tabular}{@{}lllllllllllllll@{}}

\toprule
                             & \multicolumn{14}{c}{EURLex4.3k ($\mu=15, \text{CV}=0.5$)}                                                                                                                                                                                                \\ \midrule
\multicolumn{1}{c|}{}        & \multicolumn{7}{c|}{Narrow ($|Y| \leq 2\mu$) (92.8\%)}                                                                     & \multicolumn{7}{c}{Diverse ($ |Y| > 2\mu$) (7.1\%)}                                               \\ \midrule
\multicolumn{1}{c|}{}        & P@$\mathcal{O}$ & R@$\mathcal{O}$ & F1@$\mathcal{O}$ & B@$\mu$ & \#K@$\mu$ & B@$2\mu$ & \multicolumn{1}{c|}{\#K@$2\mu$} & P@$\mathcal{O}$ & R@$\mathcal{O}$ & F1@$\mathcal{O}$ & B@$\mu$ & \#K@$\mu$ & B@$2\mu$ & \#K@$2\mu$ \\ \midrule
\multicolumn{1}{l|}{One2One} &      36.73           &       36.63          &         36.68         &   35.15      &    14.95&     22.73     & \multicolumn{1}{l|}{29.81}           &     14.27            &    14.18             &     14.23             &   25.98      &    14.80       &      16.63    &   29.75         \\
% \specialrule{0.05pt}{0pt}{0pt}
\multicolumn{1}{l|}{GROOV}   &  57.07               &  29.15               &    36.94              &   24.09      &   7.31        &    12.14      &  \multicolumn{1}{l|}{7.56}         &   71.55              &    32.03             &       43.06           &   69.06      &   13.57        &    41.42      &   17.33         \\
\multicolumn{1}{l|}{One2Seq} &   \underline{59.40}&  \underline{56.59}&    \underline{57.77}&  \underline{52.01}&  14.05         &    \underline{33.32}& \multicolumn{1}{l|}{22.36}           &   \underline{81.32}&   \underline{69.15}&   \underline{74.4}&   \underline{77.05}&     14.88      &    \underline{80.02}&    28.98        \\
\multicolumn{1}{l|}{PUSL}    &      \textbf{59.82}&     \textbf{58.07}&        \textbf{58.81}&    \textbf{54.75}&      14.56     &      \textbf{33.64}& \multicolumn{1}{l|}{22.02}           &       \textbf{83.90}&     \textbf{77.81}&      \textbf{80.28}&   \textbf{88.56}&    14.95       &     \textbf{82.29}&    28.78        \\
\midrule
                             & \multicolumn{14}{c}{AmazonCat ($\mu=5, \text{CV}=0.7$)}                                                                                                                                                                                               \\ \midrule
\multicolumn{1}{c|}{}        & \multicolumn{7}{c|}{Narrow ($|Y| \leq 2\mu$) (92.2\%)}                                                                     & \multicolumn{7}{c}{Diverse ($ |Y| > 2\mu$) (7.7\%)}                                               \\ \midrule
\multicolumn{1}{l|}{}        & P@$\mathcal{O}$ & R@$\mathcal{O}$ & F1@$\mathcal{O}$ & B@$\mu$ & \#K@$\mu$ & B@$2\mu$ & \multicolumn{1}{l|}{\#K@$2\mu$} & P@$\mathcal{O}$ & R@$\mathcal{O}$ & F1@$\mathcal{O}$ & B@$\mu$ & \#K@$\mu$ & B@$2\mu$ & \#K@$2\mu$ \\ \midrule
\multicolumn{1}{l|}{One2One} &      \underline{48.07}&      \underline{48.05}&       \underline{48.06}&    \textbf{48.37}&      5.00     &    \underline{38.58}& \multicolumn{1}{l|}{9.99}   &  52.66       &    52.63             &    52.64             &    \underline{70.90}&  5.00       &     \underline{60.26}&     10.00             \\
% \specialrule{0.05pt}{0pt}{0pt}

\multicolumn{1}{l|}{GROOV}   &   \textbf{85.52}&  \textbf{53.79}&   \textbf{62.54}&   \underline{48.33}&    2.97       &    24.34      & \multicolumn{1}{l|}{2.99}           &   \textbf{89.64}&  23.17               &  35.92      &   63.79      &    3.58       &   32.26       &     3.62       \\
\multicolumn{1}{l|}{One2Seq} &   39.05              &  36.49               &     37.50             &    38.74     &     4.71      &    30.63      & \multicolumn{1}{l|}{8.83}           &     56.38            &    \underline{54.93}&     \underline{55.58}&    64.28     &     4.97      &     57.57     &     9.90       \\
\multicolumn{1}{l|}{PUSL}    &      47.80           &      46.62           &         47.12         &    47.67&    4.91       &     \textbf{38.71}& \multicolumn{1}{l|}{9.49}           &     \underline{63.78}&       \textbf{60.00}&     \textbf{61.64}&     \textbf{74.82}&     5.00      &    \textbf{69.16}&     9.97       \\
\midrule
                             & \multicolumn{14}{c}{Wikipedia-1M ($\mu=5, \text{CV}=0.9$)}                                                                                                                                                                                               \\ \midrule
\multicolumn{1}{c|}{}        & \multicolumn{7}{c|}{Narrow ($|Y| \leq 2\mu$) (91.0\%)}                                                                     & \multicolumn{7}{c}{Diverse ($ |Y| > 2\mu$) (8.9\%)}                                               \\ \midrule
\multicolumn{1}{l|}{}        & P@$\mathcal{O}$ & R@$\mathcal{O}$ & F1@$\mathcal{O}$ & B@$\mu$ & \#K@$\mu$ & B@$2\mu$ & \multicolumn{1}{c|}{\#K@$2\mu$} & P@$\mathcal{O}$ & R@$\mathcal{O}$ & F1@$\mathcal{O}$ & B@$\mu$ & \#K@$\mu$ & B@$2\mu$ & \#K@$2\mu$ \\ \midrule
\multicolumn{1}{l|}{One2One} &         \underline{34.23}&       \underline{34.18}&       \underline{34.2}&    \underline{29.75}&    4.99       &    \textbf{20.60}& \multicolumn{1}{l|}{9.95}           &             38.24    &      \textbf{38.04}&       38.13           &  \underline{57.80}&     4.99      &     \textbf{45.94}&     9.96       \\
\multicolumn{1}{l|}{GROOV}   &     \textbf{67.04}&   \textbf{45.18}&   \textbf{52.02}&   \textbf{31.13}&    2.30       &   \underline{15.60}& \multicolumn{1}{l|}{2.31}           &     \textbf{84.79}&    26.24             &       \underline{39.2}&    \textbf{67.66}&    3.94       &    36.00      &    4.22        \\
\multicolumn{1}{l|}{One2Seq} &     23.50            &   19.91              &     21.15             &   17.69      &    3.85       &    11.27      & \multicolumn{1}{l|}{5.79}           &      \underline{45.97}&    34.76             &     38.61             &     52.85    &    4.66       &    40.16      &       8.17     \\
\multicolumn{1}{l|}{PUSL}    &      21.18          &     19.09           &     19.81             &    17.54     &     3.99     &     11.71     & \multicolumn{1}{l|}{6.26}           &           45.08      &         \underline{37.89}&      \textbf{40.37}&   53.96      &   4.79        &     \underline{42.94}&    8.75        \\
\midrule
                             & \multicolumn{14}{c}{\ourdata ($\mu=3, \text{CV}=2.8$)}                                                                                                                                                                                               \\ \midrule
\multicolumn{1}{l|}{}        & \multicolumn{7}{c|}{Narrow ($|Y| \leq 2\mu$) (91.4\%)}                                                                     & \multicolumn{7}{c}{Diverse ($ |Y| > 2\mu$) (8.5\%)}                                               \\ \midrule
\multicolumn{1}{l|}{}        & P@$\mathcal{O}$ & R@$\mathcal{O}$ & F1@$\mathcal{O}$ & B@$\mu$ & \#K@$\mu$ & B@$2\mu$ & \multicolumn{1}{l|}{\#K@$2\mu$} & P@$\mathcal{O}$ & R@$\mathcal{O}$ & F1@$\mathcal{O}$ & B@$\mu$ & \#K@$\mu$ & B@$2\mu$ & \#K@$2\mu$ \\ \midrule
\multicolumn{1}{l|}{One2One} &        35.16        &     \underline{35.14}&      \underline{35.15}&     \textbf{34.78}&       3.00    &     \textbf{24.47}& \multicolumn{1}{l|}{5.99}           &          34.44       &        \textbf{34.33}&     \textbf{34.37}&  \textbf{59.32}&      3.00     &   \textbf{48.27}&    6.00        \\
\multicolumn{1}{l|}{GROOV}   &     \textbf{54.84}&	21.77 &	28.95 &	18.72  &	1.03&	9.36  &	  \multicolumn{1}{l|}{1.03}	 &	\textbf{73.35}&   7.02	  &    12.56	&  
 26.01   &	1.07   & 	13.00	 &  1.07 \\
\multicolumn{1}{l|}{One2Seq} &    44.27	&   26.39	  &     31.26	   &     25.52	  &    1.89   &  	13.75	& \multicolumn{1}{l|}{2.17}   &	\underline{65.20}&	12.8  &	20.44    &	41.43   &	1.85  & 	22.73	&  2.10\\
\multicolumn{1}{l|}{PUSL}    &      \underline{45.72}&     \textbf{35.17}&     \textbf{38.54}&    \underline{34.50}&     2.46      &    19.48     & \multicolumn{1}{l|}{3.31}           &           60.92      &         \underline{19.51}&      \underline{27.93}&   \underline{56.11}&   2.46        &     \underline{33.75}&    3.23      \\
\midrule
\end{tabular}
\caption{Evaluation results on IID test splits across various datasets with different levels of label diversity. We report Precision@$\mathcal{O}$, Recall@$\mathcal{O}$, F1@$\mathcal{O}$, BudgetAccuracy (B@k), and number of predicted unique keyphrase (\#Keyphrases) for both the Narrow and Diverse subsets, which are divided based on the number of keyphrases per item relative to the dataset mean ($\mu$). The @$\mu$ and @$2\mu$ settings indicate the expected number of keyphrases the model should generate per item, corresponding to the average and twice the average number of keyphrases, respectively.\haoran{need to check the distribution figure again.}}
\label{tab:gtdependent}
\end{table*}

==> tables/nlp_task_example.tex <==
\begin{table*}[!htbp]
\centering
\begin{tabularx}{\textwidth}{|l|X|X|}
\hline
\textbf{NLP Task} & \textbf{Input} & \textbf{Output} \\
\hline
Joint Extraction of Relations and Entities & Albert Einstein was born in Germany and developed the theory of relativity. & head1: Albert Einstein, relation1: was born in, tail1: Germany, head2: Albert Einstein, relation2: developed, tail2: theory of relativity \\
\hline
Keyphrases Generation & MaxMara coat wool trench coat & Keyphrase1: winter coat, Keyphrase2: wool coat, ... \\
\hline
HashTag Generation & Watching the beautiful sunset over the mountains. & HashTag1: \#sunset, HashTag2: \#mountainview \\
\hline
Dataset Generation & Positive & sentence1: I love sunny days., sentence2: The beach makes me happy., ... \\
\hline
Question Generation (SQuAD) & Neil Armstrong was the first man to walk on the moon in 1969. & question: Who was the first man to walk on the moon? \\
\hline
Extreme Classification & An article discussing the evolution of reptiles during the Mesozoic era, detailing their habitats, dietary habits, and extinction events. & Label1: Paleontology, Label2: Reptiles, Label3: Mesozoic Era, Label4: Evolution, ... \\
\hline
\end{tabularx}
\caption{Examples for various NLP tasks. HashTag Generation is hard-working annotator.}
\label{tab:nlp_tasks}
\end{table*}


==> tables/pusl_vs_one2one_gt_dependent.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[!htb]
\centering
% \scriptsize
\footnotesize
% \small
% \begin{tabular}{@{}rrrrrrrrrrrrrrr@{}}
\begin{tabular}{llrr}
\toprule
Dataset & Metric & One2One & PUSL \\
\midrule
\textbf{EURLex4.3k Narrow} & B@$\mu$ & 35.15 & \textbf{54.75} \\
$\mu = 15, CV = 0.5$ & B@$2\mu$ & 22.73 & \textbf{33.64} \\
$(|Y| < 2\mu)$ (92.8\%) & F1@$O$ & 36.68 & \textbf{58.81} \\
\midrule
\textbf{EURLex4.3k Diverse} & B@$\mu$ & 25.98 & \textbf{88.56} \\
$\mu = 15, CV = 0.5$ & B@$2\mu$ & 16.63 & \textbf{82.29} \\
$(|Y| > 2\mu)$ (7.1\%) & F1@$\mathcal{O}$ & 14.23 & \textbf{80.28} \\
\midrule
\textbf{AmazonCat Narrow} & B@$\mu$ & \textbf{48.37} & 47.67 \\
$\mu = 5, CV = 0.7$ & B@$2\mu$ & 38.58 & \textbf{38.71} \\
$(|Y| < 2\mu)$ (92.2\%) & F1@$O$ & \textbf{48.06} & 47.12 \\
\midrule
\textbf{AmazonCat Diverse} & B@$\mu$ & 70.90 & \textbf{74.82} \\
$\mu = 5, CV = 0.7$ & B@$2\mu$ & 60.26 & \textbf{69.16} \\
$(|Y| > 2\mu)$ (7.7\%) & F1@$\mathcal{O}$ & 52.64 & \textbf{61.64} \\
\midrule
\textbf{\ourdata Narrow} & B@$\mu$ & \textbf{34.78} & 34.50 \\
$\mu = 3, CV = 2.8$ & B@$2\mu$ & \textbf{24.47} & 19.48 \\
$(|Y| < 2\mu)$ (91.4\%) & F1@$O$ & 35.15 & \textbf{38.54} \\
\midrule
\textbf{\ourdata Diverse} & B@$\mu$ & \textbf{59.32} & 56.11 \\
$\mu = 3, CV = 2.8$ & B@$2\mu$ & \textbf{48.27} & 33.75 \\
$(|Y| > 2\mu)$ (8.5\%) & F1@$\mathcal{O}$ & \textbf{34.37} & 27.93 \\
\bottomrule
\end{tabular}
\caption{Comparative performance of One2One and PUSL across various dataset conditions, demonstrating that PUSL often matches or surpasses One2One despite differing underlying technologies. This underscores the adaptability and effectiveness of both models across a range of dataset scenarios.}

% \caption{Comparison between One2One and PUSL across different dataset conditions. PUSL matches or exceeds One2One's performance, even though they are based on different underlying technologies. 
% % Each dataset is evaluated under specific settings with variations in average values ($\mu$) and the proportion of data falling within twice the average ($|Y|$).
% This demonstrates that both models can adapt and perform effectively across both common and varied dataset scenarios.}
\label{tab:pusl_vs_one2one_gt_dependent}
\end{table}
